FashionDPO:Fine-tune Fashion Outfit Generation Model using Direct Preference Optimization

Personalized outfit generation aims to construct a set of compatible and personalized fashion items as an outfit. Recently, generative AI models have received widespread attention, as they can generate fashion items for users to complete an incomplete outfit or create a complete outfit. However, they have limitations in terms of lacking diversity and relying on the supervised learning paradigm. Recognizing this gap, we propose a novel framework FashionDPO, which fine-tunes the fashion outfit generation model using direct preference optimization. This framework aims to provide a general fine-tuning approach to fashion generative models, refining a pre-trained fashion outfit generation model using automatically generated feedback, without the need to design a task-specific reward function. To make sure that the feedback is comprehensive and objective, we design a multi-expert feedback generation module which covers three evaluation perspectives, \ie quality, compatibility and personalization. Experiments on two established datasets, \ie iFashion and Polyvore-U, demonstrate the effectiveness of our framework in enhancing the model's ability to align with users' personalized preferences while adhering to fashion compatibility principles. Our code and model checkpoints are available at https://github.com/Yzcreator/FashionDPO.

==> sec/1_Introduction.tex <==
\section{Introduction}

Fashion in life is not merely about clothing and dressing, while it serves as a means of expressing personal style, identity, and lifestyle. 
One of the major requirements in people's daily fashion life is personalized fashion matching, where people need to pick up a set of fashion items (defined as an outfit) that are compatible with each other and fit his/her personalized fashion taste. In addition to experts in the domain of fashion, researchers in computer science demonstrate interest in studying this problem, which is defined as the task of personalized outfit recommendation. The specific tasks include obtaining a compatible fashion item based on the user's interaction history to fill an incomplete outfit—referred to as Personalized Fill-in-the-Blank (PFITB), and assembling a compatible, complete outfit for personalized recommendation.


\begin{figure}
  \includegraphics[width=0.47\textwidth]{images/task.pdf}
  % \setlength{\abovecaptionskip}{-0.2cm} 
  % \setlength{\belowcaptionskip}{-0.3cm} 
  \caption{Illustration of the motivation and paradigm comparison between FashionDPO and the supervised learning methods, where FashionDPO optimizes the model using feedback from multiple experts without relying on labelled dataset, resulting in high diversity while maintaining high quality.}
  \label{Intro-DPO}
\end{figure}

The existing works can be divided into retrieval-based and generative models.
The retrieval-based models~\cite{POG,PFOG,A-FKG,withLSTM} construct a set of personalized and compatible fashion items from the dataset. 
However, they are still limited by the variety of items in the dataset.
Currently, with the rapid development of diffusion models ~\cite{SD, controlNet}, the generative outfit recommendation (GOR) models ~\cite{CRAFT, DiFashion, OutfitGAN} have attracted widespread attention. 
Nonetheless, we found that they generate fashion items with limited diversity, failing to capture the variety of styles and preferences present in the fashion domain. Specifically, its diversity is limited by the pre-defined outfits in the dataset. For example, in the PFITB task, each incomplete outfit is paired with a unique fashion item serving as the ground truth. However, the reality is that there are multiple items that can satisfy the matching and personalization needs, but the datasest only contains one. 
Furthermore, we found that using supervised learning as the optimization objective exacerbates the limitation on diversity in pre-defined outfits.
As shown in Figure \ref{Intro-DPO}, during the training process, the generative models ~\cite{OutfitGAN,DiFashion} aim to minimize the difference between the result image and ground truth. When the generated images visually adhere to fashion compatibility but differ from ground truth, the model erroneously penalizes these deviations. This causes the model to overly focus on specific features within the pre-defined outfits, rather than learning more generalized principles of clothing compatibility, thereby limiting the diversity of the generated results.

To address the limitations of lacking diversity and supervised learning paradigm, an intuitive approach is to leverage existing solutions, such as augmenting the dataset through additional annotations. 
However, relying on human annotations can be costly, and the involvement of human annotators may introduce subjective biases into the dataset. Additionally, it becomes challenging to adapt or update the dataset when the fashion trends are constantly changing and evolving. 
A more advanced way is the RLAIF~\cite{RLAIF-sample} (reinforcement learning from AI feedback), this enables the model to learn from a variety of possible feedback and adapt to more diverse situations. This method is particularly suitable for scenarios like artistic creation, where no fixed answers exist. However, how to design the AI models to ensure that the feedback is both comprehensive and objective still remains a challenge. 
The second challenge is how to leverage the feedback generated by AI models to guide the training of generation models, which is still under-explored in the fashion domain. 
Previous method\cite{RLAIF} based on feedback typically involve first training a reward model aligned with human preferences and then fine-tuning the model using reinforcement learning. However, constructing an efficient reward model demands extensive datasets and multiple rounds of parameter tuning, which is time and resource-intensive.

To address these challenges, we propose a novel framework FashionDPO, which fine-tunes the fashion outfit generation model using direct preference optimization. 
To make sure the automatic feedbacks are comprehensive and professional, we design a multi-expert feedback generation module to address the first challenge, which consists of three experts covering diverse evaluation perspectives: 1) Quality: Evaluating whether the fashion elements in the image are complete and conform to fashion design principles. 2) Compatibility: Assessing whether the generated fashion products are coordinated within an outfit. 3) Personalization: Ensuring that the recommended fashion products align with the user's personal preferences. To solve the second challenge, we leverage the DPO~\cite{DPO} framework and define the feedback as positive-negative pairs, which are ensembled from multiple experts' feedback. We then utilize the positive-negative pairs to guide the fine-tuning process, eliminating the need to train a reward model. In summary, \textbf{the primary contributions} of our work are as follows:

\begin{itemize}[leftmargin=0.5cm, itemindent=0cm]
\item We identify the limitations of lacking diversity and supervised learning paradigm in existing personalized outfit generation models and are the first to introduce DPO framework to address the problem.

% \item We identify the limitations of lacking diversity and supervised learning paradigm in existing personalized outfit generation models and propose to leverage AI feedbacks to address the problem.

\item Fulfilling the idea of using AI feedbacks, we propose a novel framework FashionDPO, which fine-tunes the generation model using the direct preference optimization regarding multiple experts' feedbacks.

\item Extensive experiments on iFashion and Polyvore-U datasets demonstrate the effectiveness of our framework regarding various evaluating metrics.
\end{itemize}


==> sec/old_sec/1_Introduction_ver1.tex <==
\section{Introduction}

Fashion in life is not merely about clothing and dressing, while it serves as a means of expressing personal style, identity, and lifestyle. 
One of the major requirements in people's daily fashion life is personalized fashion matching, where people need to pick up a set of fashion items (defined as an outfit) that are compatible with each other and fit his/her personalized fashion taste. In addition to fashion experts, researchers in computer science define it as personalized outfit recommendation. The specific tasks include obtaining a compatible fashion item based on the user's interaction history to fill an incomplete outfit—referred to as Personalized Fill-in-the-Blank (PFITB), and assembling a compatible, complete outfit for personalized recommendation.


\begin{figure}
  \includegraphics[width=0.47\textwidth]{images/task.pdf}
  \setlength{\abovecaptionskip}{-0.2cm} 
  \setlength{\belowcaptionskip}{-0.3cm} 
  \caption{Overview of the differences between FashionDPO and supervised learning. FashionDPO optimizes the model using feedback from multiple experts, without ground truth.}
  \label{Intro-DPO}
\end{figure}



% and existing works can be divided into retrieval-based and generative models.
% The retrieval-based models~\cite{POG,PFOG,A-FKG,withLSTM} construct a set of personalized and compatible fashion items from the dataset. 
% However, they are still limited by the variety of clothing available in the dataset.
% Currently, with the rapid development of diffusion models ~\cite{SD, controlNet}, the generative model ~\cite{DiFashion}, 

% two limitations:limited diversity, misalignment between tasks and objectives

The existing works can be divided into retrieval-based and generative models.
The retrieval-based models~\cite{POG,PFOG,A-FKG,withLSTM} construct a set of personalized and compatible fashion items from the dataset. 
However, they are still limited by the variety of items in the dataset.
Currently, with the rapid development of diffusion models ~\cite{SD, controlNet}, the generative outfit recommendation (GOR) models ~\cite{CRAFT, DiFashion, OutfitGAN} have attracted widespread attention. 
Nonetheless, we found that they generate fashion items with limited diversity, failing to capture the variety of styles and preferences present in the fashion domain. Specifically, its diversity is limited by the pre-defined outfits in the dataset. For example, in the PFITB task, each incomplete outfit is paired with a unique fashion item serving as the ground truth. However, the reality is that there are multiple items that can satisfy the matching and personalization needs, but the datasest only contains one. 
%Collecting and annotating all fashion products that fit the incomplete outfit is challenging. 
% Furthermore, we found a misalignment between their tasks and objectives. Specifically, using supervised learning as the optimization objective exacerbates the limitation on diversity in pre-defined outfits.
Furthermore, we found that using supervised learning as the optimization objective exacerbates the limitation on diversity in pre-defined outfits.
As shown in Figure \ref{Intro-DPO}, during the training process, the generative models ~\cite{OutfitGAN,DiFashion} aim to minimize the difference between the result image and ground truth. When the generated images visually adhere to fashion compatibility but differ from ground truth, the model erroneously penalizes these deviations. This causes the model to overly focus on specific features within the pre-defined outfits, rather than learning more generalized principles of clothing compatibility, thereby limiting the diversity of the generated results.

%and diffusion-based model ~\cite{DiFashion,ddpm} reconstruct images from noise to closely resemble the ground truth.

% Specifically, [one sentence to summarize the first weakness]. [the following sentences to detail this aspect, through explanantion or examples]
% The existing generative fashion recommendation models ~\cite{CRAFT, DiFashion, OutfitGAN} produce fashion product images that align with design principles. 
% However, they still rely on supervised learning strategies during the training process, which is not well-suited for generative recommendation tasks.
% Specifically, in the PFITB task, each incomplete outfit is paired with a unique fashion product serving as the ground truth. However, the reality is that there are multiple clothing items that can satisfy the matching and personalization needs of an incomplete outfit, but the datasest only contains one. Collecting all fashion products that fit the incomlete outfit is very diffcult. 
% Furthermore, during the training process, GAN-based generative fashion recommendation models ~\cite{OutfitGAN} aim to minimize the difference between the generated images and the ground truth images. And diffusion-based model ~\cite{DiFashion} gradually reconstruct images from noise to closely resemble the ground truth. When the generated images visually adhere to the principles of fashion coordination but differ in detail from ground truth, the model erroneously penalizes these deviations. This can cause the model to focus excessively on 4specific features within the training data, rather than learning more generalized principles of clothing coordination, thereby limiting its ability to innovate.
% Thus, we say that supervised learning and generative fashion recommendation task are misaligned.
%To address the issues of excessive reliance on a single ground truth and the lack of flexibility in the aforementioned models, 




To address the limitations of lacking diversity and supervised learning paradigm, an intuitive approach is to leverage existing solutions, such as augmenting the dataset through additional annotations. 
However, relying on human annotations can be costly, and the involvement of human annotators may introduce subjective biases into the dataset. Additionally, it becomes challenging to adapt or update the dataset when the fashion trends are constantly changing and evolving. 
A more advanced way is the RLAIF~\cite{RLAIF-sample} (reinforcement learning from AI feedback), this enables the model to learn from a variety of possible feedback and adapt to more diverse situations. This method is particularly suitable for scenarios like artistic creation, where no fixed answers exist. However, how to design the AI models to ensure that the feedback is both comprehensive and objective still remains a challenge. 
The second challenge is how to leverage the feedback generated by AI models to guide the training of generation models, which is still under-explored in the fashion domain. 
Previous method\cite{RLAIF} based on feedback typically involve first training a reward model aligned with human preferences and then fine-tuning the model using reinforcement learning. However, constructing an efficient reward model demands extensive datasets and multiple rounds of parameter tuning, which is time and resource-intensive.

%to assure the AI feedbacks comprehensive and objective, catering to various needs in the domain of fahion

% 作为使用RLAIF的优点：As shown in Figure \ref{Intro-DPO}, we shift the learning objective from the ground truth of supervised learning to the feedback of preference models. This allows the model learn from a variety of possible outputs and adapt to more diverse situations. This approach is particularly suitable for scenarios like artistic creation, where there are no fixed answers.
%And the preference models enable the system to choose and optimize among multiple acceptable solutions.
% second challenge: Previous fine-tuning methods based on feedback typically involve first training a reward model aligned with human preferences and then fine-tuning the model using reinforcement learning. However, constructing a reward model suitable for the current task requires a large dataset and multiple rounds of parameter tuning. Thus, the second challenge is the form of feedback, specifically in how to design the reward and update mechanisms.
% Insert one paragraph here (or rewrite your original paragraph) to make the overall logic flow smooth. There is still a gap between our method and the limitations of previous works. In this paragraph, we need to present: 1) to address the limitations of lacking diversity and supervised learning paradigm, we can intuitively adopt some existing solutions, such as annotating more data. However, this is expensive if it requires human annotations, it may induce bias, and it is difficult to upgrade if the fashion trends are changing and evolving; 2) a more advanced way is the RLAIF (reinforcement learning from AI feedback). However, how to design the AI models to assure the feedbacks are more comprehensive and objective still remains a challenge. Moreover, how to leverage the feedbacks generated by AI models to supervise the training of generation models is under-explored in the fashion domain (please note here I just present the structure, you can write more details to make this paragraph complete). Then, in the next paragraph, you can start with "To address these challenges, we propose a novel framework xxx, which finetunes the fashion outfit generation model using multiple automated experts' feedbacks. Specifically, we propose a multiple experts-based feedback generation framework to address the first challenge. To solve the second challenge, we leverage the DPO framework and define the feedbacks as a binary pairs, which are ensembled from multiple experts feedback."
% To address the aforementioned issues, we propose FashionDPO, a generative fashion recommendation model based on direct preference feedback optimization. As shown in Figure \ref{Intro-DPO}, we shift the learning objective from the ground truth of supervised learning to the feedback of preference models. This allows the model learn from a variety of possible outputs and adapt to more diverse situations. This approach is particularly suitable for scenarios like artistic creation, where there are no fixed answers. And the preference models enable the system to choose and optimize among multiple acceptable solutions. However, introducing preference-based feedback learning methods in the field of fashion recommendation tasks presents the following issues: the first challenge is the need to assess the generated fashion results from multiple perspectives, which makes designing an evaluation model that accounts for these various aspects particularly difficult. Previous fine-tuning methods based on feedback typically involve first training a reward model aligned with human preferences and then fine-tuning the model using reinforcement learning. However, constructing a reward model suitable for the current task requires a large dataset and multiple rounds of parameter tuning. Thus, the second challenge is the form of feedback, specifically in how to design the reward and update mechanisms.


% To address the aforementioned issues, we propose FashionDPO, a generative fashion recommendation model based on direct preference feedback optimization.
%As shown in Figure \ref{Intro-DPO}, we shift the learning objective from the ground truth of supervised learning to the feedback of preference models.

To address these challenges, we propose a novel framework FashionDPO, which fine-tunes the fashion outfit generation model using multiple automated experts' feedbacks. To make sure the automatic feedbacks are comprehensive and professional, we design a multi-expert feedback generation module to address the first challenge, which consists of three experts covering diverse evaluation perspectives: 1) Quality: Evaluating whether the fashion elements in the image are complete and conform to fashion design principles. 2) Compatibility: Assessing whether the generated fashion products are coordinated within an outfit. 3) Personalization: Ensuring that the recommended fashion products align with the user's personal preferences. To solve the second challenge, we leverage the DPO~\cite{DPO} framework and define the feedback as binary pairs, which are ensembled from multiple experts' feedback. We then utilize the binary pairs to guide the fine-tuning process, eliminating the need to train a reward model. In summary, \textbf{the primary contributions} of our work are as follows:


% Addressing the above challenges, we integrate fashion expertise to design a comprehensive expert feedback system from three perspectives: 1) Quality: Evaluating whether the fashion elements in the image are complete and conform to fashion design principles. 2) Compatibility: Assessing whether the generated fashion products are coordinated within an outfit. 3) Personalization: Ensuring that the recommended fashion products align with the user's personal preferences. We integrated feedback from multiple experts across the aforementioned three perspectives and used it as a reward signal to fine-tune our model. Then we adopt the direct preference optimization (DPO) method for fine-tuning, which eliminates the need to train a reward model. And we utilize the data provided by the comprehensive expert feedback system to guide the learning process. In summary, \textbf{the primary contributions} of our work are as follows:


\begin{itemize}[leftmargin=0.5cm, itemindent=0cm]
 \item We identify the limitations of lacking diversity and supervised learning paradigm in GOR models, and propose multi-experts evaluation module to incorporate AI feedback.
 
 % We propose a fine-tuning framework based on multiple experts' feedback, which frees the model from the constraints of ground truth and unleashes its innovative potential.

 \item Fulfilling the idea of using AI feedback, we propose a novel framework FashionDPO, which defines the standards for  comprehensive feedback and the mechanism for its updates.
 
 % to address the challenges of limited datasets and the construction and utilization of feedback.
 %design AI evaluation models and the mechanisms for updating feedback.

 
 %We design a generative fashion products evaluation framework that incorporates fashion expertise and provides expert assessments from three perspectives: quality, compatibility, and personalization.

 \item Extensive experiments on iFashion and Polyvore-U datasets demonstrate the effectiveness of our framework improving model compatibility and personalization.
 
%In our experiments, we verify the effectiveness of the fine-tuning framework on iFashion and Polyvore-U datasets.

\end{itemize}
















































==> sec/others.tex <==
\begin{table*}[h]
\centering
\setlength{\tabcolsep}{3pt}
\caption{Performance comparison across different methods for PFITB and GOR datasets.}
\begin{tabular}{lcccccccccccccccc}
\toprule
{\#iFashion} & \multicolumn{8}{c}{PFITB} & \multicolumn{7}{c}{GOR} \\
\cmidrule(lr){2-9} \cmidrule(lr){10-16}
Methods &FID$\downarrow$ & IS$\uparrow$ & IS-acc$\uparrow$ & CS$\uparrow$ & CIS$\uparrow$ & LPIPS$\downarrow$ & Comp.$\uparrow$ & Per.$\uparrow$ & FID$\downarrow$ & IS$\uparrow$ & IS-acc$\uparrow$ & CS$\uparrow$ & CIS$\uparrow$ & LPIPS$\downarrow$ & Per.$\uparrow$ \\
\midrule
% OutfitGAN & 202.60 & 9.52 & 0.19 & 18.07 & 16.88 & 0.63 & 0.03 & 21.48 & - & - & - & - & - & - & - \\
SD-v1.5* & 52.62 & 22.54 & 0.76 & 28.30 & 38.35 & 0.68 & 0.08 & 46.31 & 38.14 & 23.20 & 0.77 & 28.46 & 55.84 & 0.69 & 46.45 \\
SD-v2* & 54.13 & 21.66 & 0.71 & \textbf{29.78} & 38.66 & 0.70 & 0.04 & 46.60 & 40.14 & 22.19 & 0.74 & \textbf{29.94} & 56.00 & 0.71 & 46.60 \\
SD-v1.5 & 42.47 & 26.76 & 0.83 & 25.67 & 44.80 & 0.62 & 0.46 & 53.16 & 28.31 & 26.90 & 0.84 & 25.62 & 63.59 & 0.63 & 53.24 \\
SD-v2 & 44.87 & 25.85 & 0.80 & 25.81 & 44.81 & 0.66 & 0.39 & 52.99 & 30.37 & 25.82 & 0.82 & 25.84 & 64.51 & 0.66 & 53.06 \\
SD-naive & 44.38 & 25.45 & 0.80 & 26.15 & 44.93 & 0.66 & 0.36 & 52.95 & 30.53 & 25.43 & 0.81 & 29.16 & 64.71 & 0.67 & 52.95 \\
ControlNet & 42.74 & 27.76 & 0.81 & 29.02 & 41.93 & 0.67 & 0.16 & 49.90 & 29.41 & 28.49 & 0.82 & 29.03 & 60.96 & 0.68 & 49.91 \\
DiFashion & 34.06 & 29.99 & 0.90 & 26.27 & 47.36 & 0.51 & 0.58 & 55.86 & 20.21 & 30.04 & 0.90 & 26.10 & 67.35 & 0.54 & 55.54 & \\
DiFashion(Lora) & \textbf{33.73} & 29.46 & 0.88 & 26.58 &  \textbf{48.33} & \textbf{0.50} & 0.59 & 55.43 & \textbf{19.40} & 30.30 & 0.90 & 26.39 & \textbf{67.68} & \textbf{0.50} & 55.89\\ 
\textbf{FashionDPO} & 38.91& \textbf{33.80} &  \textbf{0.91} &  28.41 & 45.42 & 0.53 & \textbf{0.74} & \textbf{60.39} & 23.69 & \textbf{32.37} & \textbf{0.91} & 27.97 & 64.53 & 0.53 & \textbf{59.98}\\
\bottomrule

\toprule
{\#Polyvore-U} & \multicolumn{8}{c}{PFITB} & \multicolumn{7}{c}{GOR} \\
\cmidrule(lr){2-9} \cmidrule(lr){10-16}
Methods &FID$\downarrow$ & IS$\uparrow$ & IS-acc$\uparrow$ & CS$\uparrow$ & CIS$\uparrow$ & LPIPS$\downarrow$ & Comp.$\uparrow$ & Per.$\uparrow$ & FID$\downarrow$ & IS$\uparrow$ & IS-acc$\uparrow$ & CS$\uparrow$ & CIS$\uparrow$ & LPIPS$\downarrow$ & Per.$\uparrow$ \\
\midrule
% OutfitGAN  & 272.82  & 13.63  & 0.08  & 15.08  & 23.23  & 0.70  & 0.00  & 42.59  & 16.95  & 0.73  & 50.99  \\
SD-v1.5*   & 51.34   & 17.10  & 0.73  & 27.46  & 40.56  & 0.67  & 0.70  & 51.05  & 42.59  & 16.95  & 0.73 & 27.51 & 51.68 & 0.68 & 50.99  \\
SD-v2*     & 62.41   & 14.83  & 0.68  & \textbf{29.79}  & 40.51  & 0.71  & 0.60  & 51.29  & 53.40  & 14.88  & 0.67 & \textbf{29.83} & 50.91 & 0.72 & 51.23 \\
SD-v1.5    & 53.72   & 17.12  & 0.72  & 24.31  & 45.71  & 0.64  & 0.75  &  58.20  & 44.73  &  17.24  &  0.72 &  24.34 & 58.68 & 0.65 &  58.16 \\
SD-v2      & 58.13   & 15.59  & 0.67  & 24.49  & 46.15  & 0.64  & 0.71  & 58.79  & 41.61  & 16.33  & 0.70 & 23.71 & 58.86 & 0.66 & 58.91 \\
SD-naive   & 58.22   & 15.45  & 0.66  & 24.23  & 47.01  & 0.65  & 0.73  & 59.24  & 49.04  & 15.48  &  0.67 & 24.31 & 59.18 &  0.66 & 59.12  \\
ControlNet & 44.31   & 18.93  & 0.77  & 28.67  & 43.79  & 0.68  & 0.73  & 55.44  & 36.05  & 19.21  & 0.77 & 28.72 & 56.04 &  0.69 & 55.40 \\
DiFashion  & 32.58   & 19.67  & 0.84  & 25.53  & 48.82  & 0.56  & 0.80  & 61.44  & 23.47  & 18.95  & 0.83 
 & 25.35 & 60.72 & 0.59 & 61.16\\
DiFashion(Lora)  & \textbf{30.08} & 19.75 & 0.87 & 26.01 & \textbf{49.30} & 0.54 & 0.78 & 60.38 & \textbf{23.06} & 18.69 & 0.84 & 25.96 & \textbf{60.87} & \textbf{0.55} & 60.41\\
\textbf{FashionDPO} & 34.47 & \textbf{24.14} & \textbf{0.89} &  27.26 & 45.36 & \textbf{0.55} & \textbf{0.83} & \textbf{64.67} &  28.78 & \textbf{24.93} & \textbf{0.87} & 26.14 & 55.63 & 0.58 & \textbf{64.79}\\
\bottomrule

\end{tabular}


\end{table*}

==> sec/rebuttal_www.tex <==
% review1
% (1)Although it is reasonable to introduce an external evaluation feedback mechanism to improve performance, I am concerned about the quality of the expert scoring system based on MLLM. How does the author measure whether the feedback based on MLLM is high-quality?
% (2)The entire model's training process is relatively complicated. Since no reproducible code is provided, I am concerned about the reproducibility of this work. More detailed training details need to be provided.
% (3)Do the different weights of multiple experts affect the final results?
% (4)I am concerned about the efficiency of model training and inference. The authors need to provide more detailed explanation of the efficiency.

% Rebuttal
Thanks for your constructive comments, we will provide a detailed explanation below, hoping to address your questions.
\begin{itemize}
    \item \textbf{How to measure the feedback based on MLLM is high-quality?} We also think that the expert's quality is crucial to guarantee the effectiveness of the feedback. We have overall performance evaluation study. As shown in Table 1, by introducing MLLM as the quality expert, the model's overall performance shows improvements in the IS and IS-acc metrics. Furthermore, in the ablation study, when we remove the quality expert, the results show a decline in both the IS and IS-acc metrics. 
    Because there is no such available dataset for the image quality, we cannot to do quantitative evaluation of the expert. Even with such a dataset, the dataset might not align with our goals, and ensuring the effectiveness of the dataset is also an issue. Therefore, we consider this an open problem. 
   
    
    %Firstly, we used cross-validation to analyze the model's performance. By running the MLLM model multiple times on the same input, we observed that MLLM consistently provided the same answers across different runs, indicating the consistency of the results. Secondly, we defined the task for MLLM as a classification task rather than asking it to provide a score within a range. We observed that MLLM achieved higher accuracy and result consistency in the classification task. 
    
    \item \textbf{More detailed training details.} To ensure the results are reproducible, we will release our code, dataset, and checkpoint after the paper is accepted. We have introduced a preliminary version of the implementation details in Section 5.1.3. If you are interested in any specific part of our training, you can provide further comments, and we will be happy to reply.

    % The entire training process is divided into three stages: 1) Our training subset consists of 1,000 outfits randomly selected from the iFashion and Polyvore-U dataset. During the sampling phase, we generate 7 recommended items for each outfit as a candidate set. The sampling process is divided into 50 time steps within the set {1, 2, ..., 1000}. At each time step, we save the latent variables and the noise predicted by diffusion model as data for fine-tuning. 2) We locally deploy MiniCPM to evaluate quality. For Compatibility, we train a VBPR model using paired outfit data from the POG and Polyvore-U dataset. Personalization is evaluated using the CLIP Score. Based on the score results, we categorize the preference pairs using a threshold.
    %3) If any two items from the 7 candidate generated items form a preference-non-preference relationship, we perform LoRA fine-tuning on the 50 saved timesteps. At each time step, we compute the loss and update the gradients.
    
    \item \textbf{Different weights of multiple experts.} We believe that the different weights of multiple experts will affect the final results. As shown in Table 2, when we set one of the three experts' weight to 0 and keep the others, the corresponding performance decreases, indicating that different weights have an impact on the results. But the key contribution of our paper is to propose the framework of automatically generated feedback from multiple experts to fine-tune the model. And research on different weights would consume a large amount of computational resources and time, so we assign the same weight to all three experts. In future work, we are also excited to explore this meaningful direction.

    
    %Thanks for your suggestion. We replaced the experts with a verification of the framework's generalizability and assigned equal weights to the three aspects of the experts. In future work, we plan to explore research on interactions between experts, and the weight differences between different experts, as you mentioned, is also a valuable direction for further study.

    \item \textbf{more detailed explanation of the efficiency.} The fine-tuning framework we propose is efficient. First, we achieve significant fine-tuning results with just 5 epochs. Second, we use only 1,000 outfits as training data, rather than the entire dataset. Third, we use LoRA to fine-tune the parameters in the attention layer of Stable Diffusion, while freezing the other parameters. In contrast, DiFashion trains the entire model on datasets like iFashion. We also consider efficiency to be an important issue, and there are many general techniques that can be incorporated into our approach, such as using better GPUs, reducing the timesteps required for fine-tuning, or applying acceleration techniques to improve our performance.


    
    %Our experiments were conducted on four 3090 GPUs. We analyzed the time cost in section 5.4.1. For example, if we use training subset consists of 1,000 outfits, we usually take 6 hours to sample each outfit 7 times, evaluate for 2 hours and fine-tune for 20 hours.
\end{itemize}

% MLLM was trained on large-scale data, which includes domain-specific knowledge in the Fashion field, allowing it to transfer this knowledge into our model through the judgment process.




% review2
% (1)It is compared only with one recent work, DiFashion, and may be missing some evaluation metrics. The pipeline constructed in this paper is based on DiFashion, but why are some metrics reported in the DiFashion paper missing, such as CS, CIS, and LPIPS?
% (2)The theory is empirical, requiring multiple additional models for rating and extensive training on a large number of preference pairs, which results in a high overall cost.
% (3)The superscripts and subscripts of some items are somewhat inconsistent.
% (4)Missing some details settings, such as the prompt for getting queality feedback.
% (5)For text DPO, not every token in the chosen sequence is necessarily better than those in the rejected sequence (as referenced in From r to Q∗: Your Language Model is Secretly a Q-Function, COLM 2024). Therefore, I have concerns about the validity of the assumption made in lines 515-517.
% (6)For the last few time steps in the image (t′∼T), since both itw and itl are already close to entire noise, I am concerned that contrastive learning in this context is redundant

% Rebuttal
Thanks for your constructive comments, we will provide a detailed explanation below, hoping to address your questions.
\begin{itemize}
    \item \textbf{Why we didn't use CS, CIS, and LPIPS:} We follow DiFashion [1] to compare with SD and ControlNet. At the same time, DiFashion is a well-recognized SOTA method, so there is no need to include other models. We evaluate the image generation quality using the IS and IS-acc metrics, as their computation does not require ground truth. But CS, CIS, and LPIPS are metrics that measure the difference between generated images and the ground truth, they are typically used in supervised learning. These metrics do not reflect the goals of our fine-tuning process.
    
    % Since CS, CIS, and LPIPS are metrics that measure the difference between generated images and the ground truth, they are typically used in supervised learning. However, our method is based on a feedback-based fine-tuning approach, which does not rely on ground truth. Moreover, after fine-tuning, the model exhibits stronger diversity, and these metrics do not reflect the goals of our fine-tuning process.
    \item \textbf{Overall cost:} Our model training cost is not very high. The number of epochs and the dataset required for fine-tuning are small, and we use LoRA to fine-tune only the attention layers in the U-Net. The key contribution of our work is to propose a fine-tuning framework based on multiple experts' feedback. The framework has great potential to be extended, for example, we can design different experts to fine-tune the Diffusion model according to the requirements. we can also apply general methods to improve the efficiency of our model training, such as using better GPUs, reducing the timesteps required for fine-tuning, or applying acceleration techniques.

    
    % Using DPO for fine-tuning does indeed involve computational resource consumption. In future work, we will explore ways to accelerate the fine-tuning process and eliminate redundant fine-tuning time steps.
    \item \textbf{The prompt for getting quality feedback.} We defined the task for MLLM as a classification task and used following prompt to get quality feedback: This task involves evaluating the generated fashion items. Consider whether the fashion elements in the image are complete and whether they conform to fashion design principles. The goal is to classify the quality into one of the following categories: 1-Very Poor Quality, 2-Poor Quality, 3-Low Quality, 4-Below Average Quality, 5-Moderate Quality, 6-Above Average Quality, 7-Good Quality, 8-Very Good Quality, 9-High Quality, 10-Exceptional Quality. You must reply with one of the categories exactly as listed before. Please provide the best possible category based on the available information.

    
    \item \textbf{The assumption of DPO.} We think the point you raised is valid. In this work, we follow the assumption from D3PO [2], which has been validated as effective in D3PO. This assumption is also valid in our approach. In future work, we will further explore this idea, as it may help improve the efficiency of model fine-tuning.
    
    
    % Our hypothesis follows D3PO[1], which proposed this assumption and provided related proofs: if the generated result aligns with the preference, then the predicted image at each time step also aligns with the preference.


    
    \item \textbf{Initial stage of model training.} Thanks for your insightful point. This is also a potential approach to improve the fine-tuning efficiency of the model, and we will conduct experiments to validate this in future work.

    [1] Xu, Yiyan, et al. "Diffusion Models for Generative Outfit Recommendation." Proceedings of the 47th International ACM SIGIR Conference on Research and Development in Information Retrieval. 2024.
    [2] Yang, Kai, et al. "Using human feedback to fine-tune diffusion models without any reward model." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2024.
\end{itemize}



% Reviewer3
% (1)What are the specific implementation details of the multi-expert feedback generation module? What are the specific responsibilities of each expert? How do you ensure that the feedback from these experts is comprehensive and objective? 
% (2)How are conflicting views between different experts handled during the model fine-tuning process? How does the system make a final decision if different experts assess the same sample inconsistently? 
% (3)Is there an example of the display of exotic clothing in the results generated by the model? What are the results of the generation of these bizarre garments?

% Rebuttal
Thanks for your constructive comments, we will provide a detailed explanation below, hoping to address your questions.
\begin{itemize}
    \item \textbf{Multi-expert feedback generation module.} (1) The implementation details of the multi-expert feedback generation module are introduced in Section 4.2. You can provide further comments, and we will be happy to reply.  
    (2) As mentioned in section 4.2, we locally deployed MiniCPM to evaluate quality. For Compatibility, we trained a VBPR model using paired outfit data from the POG and Polyvore-U dataset. Personalization was evaluated using the CLIP Score. Based on the score results, we categorized the preference pairs using a threshold. 
    (3) We have overall performance evaluation study in Table 1. But there is no such available dataset for the image quality, we cannot to do quantitative evaluation of each expert. The key contribution of our work is to propose a fine-tuning framework based on multiple experts' feedback. We will try to conduct experiments to demonstrate the effectiveness of the expert and include the results in the paper.

    
    
    % (1) The task of this module is to evaluate the sampled items and construct preference-non-preference pairs based on the evaluation results, which will be used in the subsequent fine-tuning process. 
    (2) As mentioned in section 4.2, we locally deployed MiniCPM to evaluate quality. For Compatibility, we trained a VBPR model using paired outfit data from the POG and Polyvore-U dataset. Personalization was evaluated using the CLIP Score. Based on the score results, we categorized the preference pairs using a threshold. 
    (3) To ensure that the feedback from these experts was comprehensive and objective, we replaced the experts with a verification of the framework's generalizability in section 5.4.2. And we conducted ablation experiments by removing one of the evaluation experts in each of three areas and fine-tuning separately. The experimental results showed that the absence of any one expert led to a decline in performance, thus demonstrating that these experts were comprehensive. To measure the feedback based on MLLM is objective, we used cross-validation to analyze the model's performance. By running the MLLM model multiple times on the same input, we observed that MLLM consistently provided the same answers across different runs, indicating the consistency of the results.
    \item \textbf{Conflicting views between different experts.} Thanks for your suggestion. Due to the length of the paper and time constraints, we did not conduct further research on this aspect. Our main goal was to validate that fine-tuning using multiple experts' feedback is effective. From the results, we can see a significant improvement in model performance. In future work, we will explore research on interactions between experts. 
    
    
    % Thanks for your suggestion. As mentioned in the future cork, we plan to explore research on interactions between experts. 
    \item \textbf{Generate results.} Even the most of the clothing images generated by our model is normal images, but our framework has potential to quickly adapt to encourage the model to generate exotic clothing images. For example, we can design an expert to give higher scores to exotic clothing, thereby introducing preference information into the model through fine-tuning. If you means the model's creativity, our framework also has the ability to encourage the model to generate more creative images only if the creativity can be quantitatively evaluated.


    %We did not observe exotic clothing in the experimental results. The generated items adhered to clothing principles and were well-coordinated within the outfits.
\end{itemize}




% Reviewer4
% Rebuttal
% (6)In the Ablation Study, what’s the difference between “w/o Feedback” and the pre-trained DiFashion?
\begin{itemize}
    \item \textbf{w/o Feedback.} As mentioned in section 5.2.2, in the case of without feedback, we modified the attention layer of the pre-trained DiFashion model and performed LoRA fine-tuning using paired data from the dataset. The difference from other ablation models is the source of fine-tuning data; other models use preference pairs from the feedback.
    \item \textbf{About notations.} 1) We have rechecked and found that in the Preliminary section, there is an inconsistency in the image parameters in our writing. We will make the necessary revisions in the subsequent version. 2) In Section 4.3, the introduction of state, action, and policy is the key component that introduces the DPO framework into the diffusion process. Both are based on Markov processes. The state $s_t$  can be viewed as the noisy image $i_t$ at time step $t$ in the diffusion process, while the action $a_t$ can be seen as the denoising process. 3) As mentioned in lines 363-365, the condition $c$ is a set of conditions $h,m,k$, so I believe it can be used to refine the formula when necessary. 4) The Feedback contains evaluations of the sampling results. Items that align with preferences are labeled as $w$, while those that do not are labeled as $l$. We compare the 7 sampling results of the same outfit pairwise. If one is labeled as $w$ and the other as $l$, it indicates a preference-non-preference relationship, which can be used for fine-tuning.
    \item \textbf{About diffusion models and DiFashion.} 1) In diffusion model, $\mu_\theta$ represents the mean of the image predicted by the U-Net network. We will make a correction in the paper. 2) Firstly, the inference process and the forward process are not mutually inclusive. I am unclear about what you mean by "the inference process in DiFashion does not involve the forward process." Secondly, as you mentioned, we use DiFashion as the sampling method, which is not one of the contributions we propose. Therefore, the details of DiFashion will be described briefly and modified.
\end{itemize}



% Reviewer5
% (1)The author's work lacks sufficient reproducibility, making it difficult to observe and verify the experimental performance in finer detail.
% (2)The author employs multiple models to serve as different experts, such as MiniCPM. However, it appears that these selections may have been made manually. It is essential for the authors to justify the rationale behind choosing these specific models as experts, as this aspect is crucial to the overall validity and effectiveness of the proposed framework.
% (3)Is the human evaluation statistically significant? I believe that having only five participants may introduce substantial bias in the results. A larger participant pool would enhance the robustness and reliability of the evaluation findings, making it crucial for the authors to address this limitation in their study.
% (4)Figure 2 is quite confusing, as it contains numerous mathematical symbols without adequate explanation. Providing an example or a more detailed description would greatly enhance clarity and help readers better understand the presented concepts.
% (5)The authors utilize a substantial number of hyperparameters, such as combining the evaluation results of multiple experts to obtain a weighted score. This raises concerns about the practicality of the approach.
% (6)The use of DPO with static data may lead to overfitting on the training dataset. Additionally, this approach could result in significant computational resource and time consumption. It would be helpful for the authors to address how they plan to mitigate these issues, such as through techniques like regularization, data augmentation, or other strategies to enhance generalization while managing resource efficiency.

% Rebuttal
Thanks for your constructive comments, we will provide a detailed explanation below, hoping to address your questions.
\begin{itemize}
    \item \textbf{More detailed training details.} The entire training process is divided into three stages: 1) Our training subset consists of 1,000 outfits randomly selected from the iFashion and Polyvore-U dataset. During the sampling phase, we generate 7 recommended items for each outfit as a candidate set. The sampling process is divided into 50 time steps within the set {1, 2, ..., 1000}. At each time step, we save the latent variables and the noise predicted by diffusion model as data for fine-tuning. 2) Based on the score results, we categorize the preference pairs using a threshold.
    3) If any two items from the 7 candidate generated items form a preference-non-preference relationship, we perform LoRA fine-tuning on the 50 saved timesteps. At each time step, we compute the loss and update the gradients.


    
    \item \textbf{The choose of experts.} The selection of experts is divided into two levels: the first is selecting which categories of experts to choose, and the second is choosing the type of model for each category. In terms of categories, we follow DiFashion and use quality, compatibility, and personalization. As for choosing which model to use in each category, we consider this an open problem, and since Multimodal Large Language Models (MLLMs) is rapidly evolving, we do not aim for absolute performance. Our goal is to provide a proof of concept. Therefore, we use as few resources as possible to validate the framework's feasibility. We believe that using more powerful MLLMs will lead to better results, which is also part of the deeper follow-up work we plan to do in the future.

    



    
    
    To ensure that the feedback from these experts was comprehensive and objective, we replaced the experts with a verification of the framework's generalizability in section 5.4.2. And we conducted ablation experiments by removing one of the evaluation experts in each of three areas and fine-tuning separately. The experimental results showed that the absence of any one expert led to a decline in performance, thus demonstrating that these experts were comprehensive. To measure the feedback based on MLLM is objective, we used cross-validation to analyze the model's performance. By running the MLLM model multiple times on the same input, we observed that MLLM consistently provided the same answers across different runs, indicating the consistency of the results.
    \item \textbf{Human evaluation.} We invite professional fashion designers to conduct expert-level human evaluation. Since they have received professional training, their ratings are more stable. In contrast, DiFashion uses many ordinary people for evaluations. While using a large number of ordinary people may have statistical significance, the average reliability is not very high. Since professional fashion designers are scarce and their fees are relatively high, we invite 5 experts to conduct the human evaluation.







    
    
    
    Thanks for your suggestion. We will introduce more fashion designers for professional assessments and incorporate the perspective of ordinary users. 


    
    \item \textbf{Hyperparameters in multi-experts' evaluation.} As mentioned in section 5.1.3, we assigned equal weights to the three aspects of the experts. In ablation study, we also demonstrate the impact of removing a specific expert, and the results show that the current combination with equal weights is already sufficient to prove the effectiveness of the framework. In future work, we plan to eliminate the use of this hyperparameter and explore research on the interactions between experts.
    
    We assigned equal weights to the three aspects of the experts. In future work, we plan to eliminate the use of this hyperparameter and explore research on the interactions between experts.
    \item \textbf{The use of DPO.} Thanks for your insightful point. In our future work, we will explore methods to improve efficiency, such as shortening the number of time steps required for fine-tuning.
\end{itemize}
